Meta-Learning to Compositionally Generalize

Natural language is compositional; the meaning of a sentence is a function of the meaning of its parts. This property allows humans to create and interpret novel sentences, generalizing robustly outside their prior experience. Neural networks have been shown to struggle with this kind of generalization, in particular performing poorly on tasks designed to assess compositional generalization (i.e. where training and testing distributions differ in ways that would be trivial for a compositional strategy to resolve). Their poor performance on these tasks may in part be due to the nature of supervised learning which assumes training and testing data to be drawn from the same distribution. We implement a meta-learning augmented version of supervised learning whose objective directly optimizes for out-of-distribution generalization. We construct pairs of tasks for meta-learning by sub-sampling existing training data. Each pair of tasks is constructed to contain relevant examples, as determined by a similarity metric, in an effort to inhibit models from memorizing their input. Experimental results on the COGS and SCAN datasets show that our similarity-driven meta-learning can improve generalization performance.

==> figures/kernel_tree_examples.tex <==
\begin{figure}

    
\Tree [.sell liam [.box garden ] lincoln ] \\

\circled{\Tree [.sell liam ]}
\circled{\Tree [.sell box ]}
\Tree [.sell [.box garden ] ]
\Tree [.sell lincoln ] \\


\Tree [.sell liam [.box [.cabinet *monkey ] ] william ] \\

\circled{\Tree [.sell liam ]}
\circled{\Tree [.sell box ]}
\Tree [.sell [.box cabinet ] ]
\Tree [.sell [.box [.cabinet *monkey ] ] ]
\Tree [.sell william ]
\caption{The dependency trees for two sentences `Liam sold a box on a cabinet beside the monkey to William .' and "Liam sold the box in a garden to Lincoln ." Shown below each tree are that example's partial trees. As there are two two partial trees shared by the examples their un-normalized tree kernel score is 2}
\label{figure:partial-trees}
%\appendix
\end{figure}

==> sections/abstract.tex <==


\section{Abstract}

Increasingly meta-learning approaches offer a method for improving a model's generalization ability in a few-shot or zero-shot setting. Recent work has focused on applying these approaches specifically to the problem of domain generalization. Central to these approaches is the design of tasks on which meta-learning is performed, particularly when the tasks are produced by sub-sampling the existing training data. Previous work in this area has looked at sub-sampling training data in order to simulate the divergence between the source and target domains. While this has proved effective in some cases it requires prior knowledge of the target domain. Here we propose a more general-purpose method, utilizing kernels to determine the relative similarity of examples sampled into meta-tasks. We apply this novel approach to data-sets that frame the problem of compositional generalization as one of domain generalization; using string and tree kernels to select examples for each meta-task.  Experimental results on the COGS and SCAN datasets show that in some cases kernel-driven meta-learning improves the performance of a baseline model.


Natural language is  compositional, the meaning of a sentence is a function of the meaning of its parts. This property allows humans to create and interpret novel sentences, generalizing robustly outside their prior experience. Neural networks have been shown to struggle with this kind of generalization, failing to compositionally apply what they have learned. A number of datasets have been designed to assess models' compositional ability by having different distributions for training Meta-learning approaches offer a method for improving a model's generalization ability in few-shot or zero-shot settings. Recent work has focused on applying these approaches to the problem of domain generalization. Central to this work is the design of tasks on which meta-learning is performed, particularly when the tasks are produced by sub-sampling the existing training data. Previous work in this area has looked at sub-sampling training data in order to simulate the divergence between the source and target domains. While this has proved effective in some cases it requires prior knowledge of the target domain. Here we propose a more general-purpose method, utilizing kernels to determine the relative similarity of examples sampled into meta-tasks. We apply this novel approach to datasets that frame the problem of compositional generalization in natural language as one of domain generalization, using string and tree kernels to select examples for each meta-task.  Experimental results on the COGS and SCAN datasets show that kernel-driven meta-learning can improve generalization performance.


==> tables/methods_kernel_examples.tex <==
\begin{table}[t!]
  \centering
    \resizebox{\columnwidth}{!}{ 
      \begin{tabular}{lr}
    \multicolumn{2}{c}{\textbf{Source Example}:The girl was lended the balloon by Harper .} \\
      \\
      \toprule
      Neighbours using Tree Kernel & Similarity\\
      \hline
The girl lended the sailor the balloon . & 0.55 \\
The balloon was lended to Sophia by the girl . & 0.45 \\
A banana was lended to the girl . & 0.37 \\
The girl was lended a donut . & 0.37 \\
The girl was lended the chair . & 0.37 \\
       \\
        Neighbours using String Kernel\\
       \hline
The girl was lended the cake by Lucas . & 0.35 \\
The girl was lended the chair . & 0.31 \\
The coach was lended the balloon . & 0.31 \\
The girl was lended the donut . & 0.31 \\
The girl lended the sailor the balloon . & 0.31 \\
      \\
      Neighbours using LevDistance & \\
      \hline
The girl was lended the cake by Lucas . & -2.00 \\
The student was lended the sweetcorn by Emma . & -3.00 \\
The girl was lended a clock by Mia . & -3.00 \\
The girl was served the pen by Emma . & -3.00 \\
The girl was given the bag by Liam . & -3.00 \\
      \bottomrule
      \end{tabular}
  }
  \caption{Top scoring examples according to the tree kernel, string kernel and Levenshtein distance for the sentence `The sailor dusted the boy' and accompanying scores.}
  \label{table:kernel-examples}
  \end{table}
